Teach-to-Reason: Competition-Guided Reasoning with a Self-Improving Teacher

Chest X-ray visual question answering (CXR VQA) requires models not only to predict correct answers, but also to produce reliable medical reasoning. However, existing reinforcement-learning-based training typically relies on answer-level rewards, which are often too coarse to improve chain-of-thought (CoT) quality and can become ineffective when group-level advantages collapse to zero. We propose \textbf{Teach-to-Reason (T2R)}, a framework that introduces comparison-based supervision into CoT optimization through a self-improving \emph{Teacher} and a competition-guided \emph{Reasoner}. As the Teacher is iteratively strengthened via self-competition, the Reasoner is optimized against progressively stronger Teacher-generated references. We further introduce a case-wise reward design that preserves the original reward-induced positive/negative partition when it is informative, and restores supervision from competition scores when the original reward signal degenerates. Experiments on multiple CXR open-ended VQA benchmarks show that T2R consistently outperforms strong baselines, indicating that comparison-based supervision, when integrated in a controlled and principled manner, provides a more effective training signal for reasoning optimization.

==> tables/frozen_teacher_ablation.tex <==
\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{3.8pt}
\renewcommand{\arraystretch}{0.98}

\caption{Ablation on the Teacher in Frozen Teacher Experiment.}
\label{tab:frozen_teacher_stage}

\begin{tabular}{
l
*{6}{S[table-format=2.2]}
}
\toprule
\textbf{Teacher}
& \multicolumn{1}{c}{\textbf{Med-CXR}}
& \multicolumn{1}{c}{\textbf{VQA-RAD}}
& \multicolumn{1}{c}{\textbf{SLAKE}}
& \multicolumn{1}{c}{\textbf{MIMIC-CXR}}
& \multicolumn{1}{c}{\textbf{Pneumonia}}
& \multicolumn{1}{c}{\textbf{CXR-PA}} \\
\midrule
$\mathcal{T}_0$ & \second{21.74} & \multicolumn{1}{c}{\best{40.37}} & \second{52.35} & \multicolumn{1}{c}{\best{20.88}} & \multicolumn{1}{c}{\best{76.44}} & \second{40.20} \\
$\mathcal{T}_1$ & \multicolumn{1}{c}{\best{23.78}} & \second{37.50} & 51.30 & \second{19.70} & \second{67.30} & \multicolumn{1}{c}{\best{44.88}} \\
$\mathcal{T}_2$ & 18.03 & 32.19 & \multicolumn{1}{c}{\best{55.49}} & 13.57 & 35.57 & 25.14 \\
$\mathcal{T}_3$ & 17.52 & 33.33 & 51.30 & 13.31 & 37.50 & 24.26 \\
\bottomrule
\end{tabular}
\end{table}
